Automated Detection of Coronary Artery Stenosis in X-ray Angiography using Deep Neural Networks

Coronary artery disease leading up to stenosis, the partial or total blocking of coronary arteries, is a severe condition that affects millions of patients each year. Automated identification and classification of stenosis severity from minimally invasive procedures would be of great clinical value, but existing methods do not match the accuracy of experienced cardiologists, due to the complexity of the task. Although a number of computational approaches for quantitative assessment of stenosis have been proposed to date, the performance of these methods is still far from the required levels for clinical applications. In this paper, we propose a two-step deep-learning framework to partially automate the detection of stenosis from X-ray coronary angiography images. In the two steps, we used two distinct convolutional neural network architectures, one to automatically identify and classify the angle of view, and another to determine the bounding boxes of the regions of interest in frames where stenosis is visible. Transfer learning and data augmentation techniques were used to boost the performance of the system in both tasks. We achieved a 0.97 accuracy on the task of classifying the Left/Right Coronary Artery (LCA/RCA) angle view and 0.68/0.73 recall on the determination of the regions of interest, for LCA and RCA, respectively. These results compare favorably with previous results obtained using related approaches, and open the way to a fully automated method for the identification of stenosis severity from X-ray angiographies.

==> Sections/2_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
Coronary artery disease (CAD), characterized by plaque buildup inside the coronary arteries, is the leading non-communicable disease in global mortality. This buildup leads to stenosis, the partially or totally blocking of blood flow in the coronary arteries leading to improper delivery of oxygen-rich blood to the heart, weakening the heart muscle and possibly leading to heart failure. Current standard diagnostic methods rely on an expert physician to assess the case, off or on-site, using non-invasive or invasive procedures \cite{Bio:CADd,Coro:stat}. Although several resources have been invested in prevention, proper available computer-assisted assessment and treatment procedures are still not available.

%We contribute a new curated medical dataset of X-ray invasive coronary angiography labeled with optimal interval frames and annotated with stenosis bounding boxes and its respective quantitative instantaneous wave-free ratio (iFR) severity assessment measure, providing a path for novel implementations of automatic stenosis assessment. Additionally, a two-step framework based on deep neural networks is presented for coronary angle view selection and stenosis detection.

==> Sections/8_FutureWork.tex <==
\section{Future Work}
\label{section:future}
With possible incoming segmentation annotations of stenosis and coronary arteries, new novel experiments can be made, e.g automatically segment and classify the regions of interest obtained from the bounding boxes. Attention mechanisms are being increasingly developed and published in literature demonstrating its applications in all fields of research. These can be explored for iFR estimates since the stenosis only represents a small portion of the frame and these mechanisms could aid the model to learn that these are the specific regions that contribute the most to the iFR assessment.
